Translation Quality Assessment: A Brief Survey on Manual and Automatic Methods

To facilitate effective translation modeling and translation studies, one of the crucial questions to address is how to assess translation quality. From the perspectives of accuracy, reliability, repeatability and cost, translation quality assessment (TQA) itself is a rich and challenging task. In this work, we present a high-level and concise survey of TQA methods, including both manual judgement criteria and automated evaluation metrics, which we classify into further detailed sub-categories. We hope that this work will be an asset for both translation model researchers and quality assessment researchers. In addition, we hope that it will enable practitioners to quickly develop a better understanding of the conventional TQA field, and to find corresponding closely relevant evaluation solutions for their own needs. This work may also serve inspire further development of quality assessment and evaluation methodologies for other natural language processing (NLP) tasks in addition to machine translation (MT), such as automatic text summarization (ATS), natural language understanding (NLU) and natural language generation (NLG).

==> fig-xx-steps.tex <==
% 9168896
%Rxd3: INFO:tensorflow:Total trainable variables size: 80288000
%Rxd2: INFO:tensorflow:Total trainable variables size: 80591104


%Total trainable variables size


{\centering
% empty line required
\begin{tikzpicture}
%\begin{center}
\begin{axis}
%\begin{center}
[%
graph,
height=\graphheight,
width=\graphwidth,
xlabel=Learning Steps,
ylabel=BLEU scores,
ymin=11,
legend style={
cells={anchor=west},
%legend pos=south east,
style={at={(0.957,0.8)}}
}
]
\pgfplotstableread[col sep=comma]{zh2en_NMT_BLEU_scores.txt}\plotdata

\addplot[color=aqua,mark=triangle] table[x=models, y=baseline] {\plotdata};
\addlegendentry{\textsc{base}}

\addplot[color=blue,mark=*] table[x=models, y=rxd1] {\plotdata};
\addlegendentry{\textsc{rxd1}}

\addplot[color=black,mark=o] table[x=models, y=rxd2] {\plotdata};
\addlegendentry{\textsc{rxd2}}

\addplot[color=red,mark=square] table[x=models, y=rxd3] {\plotdata};
\addlegendentry{\textsc{rxd3}}

\addplot[color=yellow,mark=diamond] table[x=models, y=rxd3+MWE] {\plotdata};
\addlegendentry{\textsc{rxd3}MWE}
%https://tex.stackexchange.com/questions/134346/different-marker-shape-for-pgf-tikz

%\end{center}
\end{axis}
%\end{center}
\end{tikzpicture}
% empty line required

}

==> sec-further-discussion.tex <==


So far, the human judgment scores of MT results are usually considered as the golden standard that the automatic evaluation metrics should try to approach. However, some improper handlings in the process also yield problems. For instance, in the ACL WMT 2011 English-Czech task, the multi-annotator agreement kappa value k is very low and even the exact same string produced by two systems is ranked differently each time by the same annotator. The evaluation results are highly affected by the manual reference translations. How to ensure the quality of reference translations and the agreement level of human judgments are two important problems.

Automatic evaluation metrics are indirect measures of translation quality, because that they are usually using the various string distance algorithms to measure the closeness between the machine translation system outputs and the manually offered reference translations and they are based on the calculating of correlation score with manual MT evaluation \cite{MoranLewis2012}. Furthermore, the automatic evaluation metrics tend to ignore the relevance of words \cite{Koehn2010}, for instance, the name entities and core concepts are more important than punctuations and determiners but most automatic evaluation metrics put the same weight on each word of the sentences. Third, automatic evaluation metrics usually yield meaningless score, which is very test set specific and the absolute value is not informative. For instance, what is the meaning of -16094 score by the MTeRater metric \cite{PartonTetreaultMadnani2011} or 1.98 score by ROSE \cite{SongCohn2011}? 
And similar goes to 19.07 by BEER / 28.47 by BLEU / 33.03 by METEOR for a mostly good translation in the paper (see experiments section Table 4) \cite{MaillettedeBuyWenniger2015}? Instead, we find one interesting metric family LEPOR and hLEPOR \cite{HanWongChao2012,han2014lepor} that can give a somehow meaningful score for a somehow recognized good translation, e.g. the score can be around 0.60 to 0.80.

%And 19.07 by BEER / 28.47 by BLEU / 33.03 by METEOR for a mostly good translation? (Gideon MT paper, table 4)\cite{MaillettedeBuyWenniger2015}. Instead, we find one interesting metric LEPOR that can give a 
The automatic evaluation metrics should try to achieve the goals of low cost, reduce time and money spent on carrying out evaluation; tunable, automatically optimize system performance towards metric;meaningful, score should give intuitive interpretation of translation quality;consistent, repeated use of metric should give same results;correct, metric must rank better systems higher as mentioned in \cite{Koehn2010}, of which the low cost, tunable and consistent characteristics are easily achieved by the metric developers, but the rest two goals (meaningful and correct) are usually the challenges in front of the NLP researchers.

There are some related works about MT evaluation survey or literature review before. For instance, in the DARPA GALE report \cite{GALEprogram2009}, researchers first introduced the automatic and semi-automatic MT evaluation measures, and the task and human in loop measures; then, they gave a description of the MT metrology in GALE program, which focus on the HTER metric as standard method used in GALE; finally, they compared some automatic metrics and explored some other usages of the metric, such as optimization in MT parameter training.

In another research project report EuroMatrix \cite{EuroMatrixProject2007}, researchers first gave an introduction of the MT history, then, they introduced human evaluation of MT and objective evaluation of MT as two main sections of the work; finally, they introduced a listed  of popular evaluation measures at that time including WER, SER, CDER, X-Score, D-score, NIST, RED, IER and TER etc. 

% (grave accent): enter image description here
M$\grave{a}$rquez \newcite{Marquez2013talk} introduced the Asiya online interface developed by their institute for MT output error analysis, where they also briefly mentioned the MT evaluation developments of lexical measures and linguistically motivated measures, and pointed out the the challenges in the quality estimation task.
%Màrquez \cite{Marquez2013talk} introduced the Asiya online interface developed by their institute for MT output error analysis, where they also briefly mentioned the MT evaluation developments of lexical measures and linguistically motivated measures, and pointed out the the chanllenges in the quality estimation task.


Our work differs with the previous ones, by introducing some recent development of MT evaluation models,  the different classifications from manual to automatic evaluation measures, the introduction of recent QE tasks, and the concise construction of the content.
